Abstract Family-based Model Checking using Modal Featured Transition Systems: Preservation of CTL* (Extended Version)

Variational systems allow effective building of many custom variants by using features (configuration options) to mark the variable functionality. In many of the applications, their quality assurance and formal verification are of paramount importance. Family-based model checking allows simultaneous verification of all variants of a variational system in a single run by exploiting the commonalities between the variants. Yet, its computational cost still greatly depends on the number of variants (often huge). In this work, we show how to achieve efficient family-based model checking of CTL* temporal properties using variability abstractions and off-the-shelf (single-system) tools. We use variability abstractions for deriving abstract family-based model checking, where the variability model of a variational system is replaced with an abstract (smaller) version of it, called modal featured transition system, which preserves the satisfaction of both universal and existential temporal properties, as expressible in CTL*. Modal featured transition systems contain two kinds of transitions, termed may and must transitions, which are defined by the conservative (over-approximating) abstractions and their dual (under-approximating) abstractions, respectively. The variability abstractions can be combined with different partitionings of the set of variants to infer suitable divide-and-conquer verification plans for the variational system. We illustrate the practicality of this approach for several variational systems.

==> conclusion.tex <==

We have proposed variability abstractions to derive abstract model checking for families of
related systems. The abstractions
are applied before model generation directly on \fpromela\,
programs. % as source to source transformations.
The evaluation confirms that interesting properties can be efficiently verified in this way
by only a few calls to $\spin$.
